Contextualized Evaluations: Judging Language Model Responses to Underspecified Queries

Language model users often issue queries that lack specification, where the context under which a query was issued -- such as the user's identity, the query's intent, and the criteria for a response to be useful -- is not explicit. For instance, a good response to a subjective query like "What book should I read next?" would depend on the user's preferences, and a good response to an open-ended query like "How do antibiotics work against bacteria?" would depend on the user's expertise. This makes evaluation of responses to such queries an ill-posed task, as evaluators may make arbitrary judgments about the response quality. To remedy this, we present contextualized evaluations, a protocol that synthetically constructs context surrounding an underspecified query and provides it during evaluation. We find that the presence of context can 1) alter conclusions drawn from evaluation, even flipping benchmark rankings between model pairs, 2) nudge evaluators to make fewer judgments based on surface-level criteria, like style, and 3) provide new insights about model behavior across diverse contexts. Specifically, our procedure suggests a potential bias towards WEIRD (Western, Educated, Industrialized, Rich and Democratic) contexts in models' "default" responses and we find that models are not equally sensitive to following different contexts, even when they are provided in prompts.

==> sections/_hedging.tex <==
To understand how models respond to these underspecified queries, we generate responses to these queries using multiple models,\footnote{The method for sampling underspecified queries and model identities are mentioned in \S\ref{subsec:generating_context}.} then randomly sample one response and label it into one of six response types listed in Table~\ref{tab:response_types} using \texttt{GPT-4o}.

\input{tables/response_types}

We find that models are prone to hedging against uncertainty when posed with underspecified queries, concurring with prior work \cite{herlihy2024overcoming}. For instance, for a query such as "\textit{Come up with easy dinner ideas for weeknights}", where context about the user and their preferences is unknown, a typical model response might address multiple possible dietary preferences in a lengthy manner. While this may be a reasonable strategy, it also has downstream implications for evaluation. 

==> tables/constraints_satisfied.tex <==
\renewcommand{\arraystretch}{1.2}

% \begin{table*}[t!]
%     \centering
%     \scalebox{.85}{
%     \setlength\tabcolsep{4pt}
%     \begin{tabular}{>{\raggedright\arraybackslash}m{5cm}ccc|ccc}
%         \toprule
%         \multirow{2}{*}{Model Pair} & \multicolumn{3}{c}{\texttt{NoCtxGen-CtxEval}} & \multicolumn{3}{c}{\texttt{CtxGen-CtxEval}} \\ 
%         \cline{2-7} \addlinespace[1mm]
%          & \makecell{1} & \makecell{2} & |Avg Diff.| & \makecell{1} & \makecell{2} & |Avg Diff.| \\
%          \midrule
%         \texttt{GPT-4o vs Gemini-1.5-Flash} & 5.29 & 5.14 & 1.33 & 7.69 & 7.40 & 1.01 \\
%         \texttt{Claude-3.5-Sonnet vs Llama-3.1-405B} & 5.40 & 5.29 & 1.64 & 8.03 & 7.61 & 0.96  \\
%         \texttt{Gemma-2-27B vs Jamba-1.5-Large} & 4.55 & 4.96 & 1.91 & 7.27 & 7.46 & 1.06 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Average number of constraints satisfied by different model pairs in context-aware evaluation settings. Shown here are the total number of follow-up QAs which are satisfied by candidate 1 and candidate 2 (in the order listed in the first column), as well as their absolute average difference. We note that the ability of models to follow instructions in the context varies.}
%     % \vspace{-5pt}
%     \label{tab:constraints_satisfied}
% \end{table*}



\begin{table*}[t]
    \centering
    % Subtable for GPT-4o and Gemini-1.5-Flash
    \begin{subtable}[t]{0.9\linewidth}
        \centering
        \scalebox{.85}{
        \setlength\tabcolsep{4pt}
        \begin{tabular}{l ccc}
            \toprule
            Condition & GPT-4o & Gemini-1.5-Flash & \(|\mathrm{Avg\,Diff.}|\) \\
            \midrule
            \texttt{NoCtxGen-CtxEval} & 5.29 & 5.14 & 1.33 \\
            \texttt{CtxGen-CtxEval}    & 7.69 & 7.40 & 1.01 \\
            \bottomrule
        \end{tabular}
        }
        % \caption{GPT-4o and Gemini-1.5-Flash}
    \end{subtable}
    
    \vspace{1em} % vertical space as separator
    
    % Subtable for Claude-3.5-Sonnet and Llama-3.1-405B
    \begin{subtable}[t]{0.9\linewidth}
        \centering
        \scalebox{.85}{
        \setlength\tabcolsep{4pt}
        \begin{tabular}{l ccc}
            \toprule
            Condition & Claude-3.5-Sonnet & Llama-3.1-405B & \(|\mathrm{Avg\,Diff.}|\) \\
            \midrule
            \texttt{NoCtxGen-CtxEval} & 5.40 & 5.29 & 1.64 \\
            \texttt{CtxGen-CtxEval}    & 8.03 & 7.61 & 0.96 \\
            \bottomrule
        \end{tabular}
        }
        % \caption{Claude-3.5-Sonnet and Llama-3.1-405B}
    \end{subtable}
    
    \vspace{1em} % vertical space as separator
    
    % Subtable for Gemma-2-27B and Jamba-1.5-Large
    \begin{subtable}[t]{0.9\linewidth}
        \centering
        \scalebox{.85}{
        \setlength\tabcolsep{4pt}
        \begin{tabular}{l ccc}
            \toprule
            Condition & Gemma-2-27B & Jamba-1.5-Large & \(|\mathrm{Avg\,Diff.}|\) \\
            \midrule
            \texttt{NoCtxGen-CtxEval} & 4.55 & 4.96 & 1.91 \\
            \texttt{CtxGen-CtxEval}    & 7.27 & 7.46 & 1.06 \\
            \bottomrule
        \end{tabular}
        }
        % \caption{Gemma-2-27B and Jamba-1.5-Large}
    \end{subtable}
    
    \caption{Average number of constraints satisfied by different model pairs in context-aware evaluation settings. Shown here are the total number of follow-up QAs that are satisfied by each candidate (named directly) as well as the absolute average difference.}
    \label{tab:constraints_satisfied}
\end{table*}

==> tables/human_agreement.tex <==
\definecolor{lightgreen}{RGB}{204, 255, 204} % Light green for lower values
\definecolor{mediumgreen}{RGB}{102, 255, 102} % Medium green
\definecolor{darkgreen}{RGB}{0, 204, 0} % Dark green for higher values

\definecolor{lblue}{RGB}{204, 229, 255} % Light blue for lower kappa values
\definecolor{mblue}{RGB}{102, 178, 255} % Medium blue
\definecolor{dblue}{RGB}{0, 102, 204} % Dark blue for higher kappa values

\renewcommand{\arraystretch}{1.25} % Default value: 1

% Agreement conditional formatting (green gradient)
\newcommand{\colorcellhumanagreement}[1]{%
  \ifdim#1pt<70pt\cellcolor{lightgreen}#1\else%
  \ifdim#1pt<75pt\cellcolor{mediumgreen}#1\else%
  \cellcolor{darkgreen}#1\fi\fi}

\begin{table*}[t!]
    \centering
    \scalebox{0.8}{
    \setlength\tabcolsep{4pt}
    \begin{tabular}{>{\raggedright\arraybackslash}m{5cm}c|c|c}
        \toprule
        \multirow{2}{*}{Model Pair} & \multicolumn{1}{c}{\texttt{NoCtxGen-NoCtxEval}} & \multicolumn{1}{c}{\texttt{NoCtxGen-CtxEval}} & \multicolumn{1}{c}{\texttt{CtxGen-CtxEval}} \\ 
        \cline{2-4} \addlinespace[1mm] % Adds vertical space after cline
         & \makecell{Agreement \% \\w/ ties (w/o ties)} & \makecell{Agreement \% \\w/ ties (w/o ties)} & \makecell{Agreement \% \\w/ ties (w/o ties)} \\
         \midrule
        \texttt{GPT-4o} vs \texttt{Gemini-1.5-Flash} & \colorcellhumanagreement{70.67} (73.33) & \colorcellhumanagreement{75.00} (77.15) & \colorcellhumanagreement{76.00} (76.36) \\
        \texttt{Claude-3.5-Sonnet} vs \texttt{Llama-3.1-405B} & \colorcellhumanagreement{65.99} (67.75) & \colorcellhumanagreement{71.33} (72.84) & \colorcellhumanagreement{74.67}\sym{*} (77.19\sym{*}) \\
        \texttt{Gemma-2-27B} vs \texttt{Jamba-1.5-Large} & \colorcellhumanagreement{71.33} (73.95) & \colorcellhumanagreement{74.00} (75.48) & \colorcellhumanagreement{75.33} (75.79) \\
        \bottomrule
    \end{tabular}
    }
    \caption{Human agreement statistics for different model pairs in all three evaluation settings. Note that the agreement is slightly higher for a subset of model pairs.}
    % \vspace{-10pt}
    \label{tab:human_agreement}
\end{table*}

==> tables/human_win_rates.tex <==
\renewcommand{\arraystretch}{1.2}

\begin{table*}[t!]
    \centering
    \scalebox{.85}{
    \setlength\tabcolsep{4pt}
    \begin{tabular}{>{\raggedright\arraybackslash}m{5cm}ccc|ccc|ccc}
        \toprule
        \multirow{2}{*}{Model Pair} & \multicolumn{3}{c}{\texttt{NoCtxGen-NoCtxEval}} & \multicolumn{3}{c}{\texttt{NoCtxGen-CtxEval}} & \multicolumn{3}{c}{\texttt{CtxGen-CtxEval}} \\ 
        \cline{2-10} \addlinespace[1mm]
         & \makecell{1} & \makecell{2} & Tie & \makecell{1} & \makecell{2} & Tie & \makecell{1} & \makecell{2} & Tie  \\
         \midrule
        \texttt{GPT-4o vs Gemini-1.5-Flash} & 40.24 & \textbf{48.78} & 10.98 & 40.86 & \textbf{50.54} & 8.60 & \textbf{52.75} & 32.97 & 14.29 \\
        \texttt{Claude-3.5-Sonnet vs Llama-3.1-405B} & \textbf{58.75} & 37.50 & 3.75 & \textbf{45.88} & 36.47 & 17.65 & \textbf{55.55} & 24.44 & 20.00 \\
        \texttt{Gemma-2-27B vs Jamba-1.5-Large} & 38.82 & \textbf{54.12} & 7.06 & 36.67 & \textbf{50.00} & 13.33 & \textbf{49.43} & 34.48 & 16.09 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Win rates based on the majority human vote, for all model pairs and evaluation settings. Shown here are the win rates of candidate 1, candidate 2 (in the order listed in the first column) and their tie rate. Note that the preferred model (with a higher win rate) can vary across context-agnostic and context-aware settings.}
    \vspace{-10pt}
    \label{tab:human_win_rates}
\end{table*}

==> tables/response_types.tex <==
\renewcommand{\arraystretch}{1.4} % Default value: 1
\definecolor{Lavender}{rgb}{0.9,0.9,0.98}

\begin{table}[t!]
\centering
\scalebox{.7}{
\begin{tabular}{ >{\raggedright\arraybackslash}p{3.5cm} p{5cm} c }
\rowcolor{Lavender!40}
 \textbf{Response Type} & \textbf{Description} & \textbf{\%} \\ \toprule
\textsc{Direct Response} & Respond to the query assuming a specific context & \cellcolor{blue!25} 5.32 \\
\textsc{Hedging} & Respond to the query for multiple contexts with further explanation & \cellcolor{blue!60} 82.40 \\
\textsc{Direct Response + Follow-Up} & Respond to the query assuming a specific context \& ask a follow-up question & \cellcolor{blue!15} 0.58 \\
\textsc{Hedging + Follow-Up} & Respond to the query for multiple contexts with further explanation \& ask a follow-up question & \cellcolor{blue!40} 9.62 \\
\textsc{Follow-Up} & Only ask a follow-up question & \cellcolor{blue!20} 0.80 \\
\textsc{Refusal} & Refuse to answer altogether & \cellcolor{blue!20} 1.28 \\
 \bottomrule
\end{tabular}
}
\caption{Models are prone to hedging against uncertainty in underspecified queries by generating a long response corresponding to multiple contexts.}
\label{tab:response_types}
\vspace{-10pt}
\end{table}
